Distribution of Action Movements (DAM): A Descriptor for Human Action Recognition

Human action recognition from skeletal data is an important and active area of research in which the state of the art has not yet achieved near-perfect accuracy on many well-known datasets. In this paper, we introduce the Distribution of Action Movements Descriptor, a novel action descriptor based on the distribution of the directions of the motions of the joints between frames, over the set of all possible motions in the dataset. The descriptor is computed as a normalized histogram over a set of representative directions of the joints, which are in turn obtained via clustering. While the descriptor is global in the sense that it represents the overall distribution of movement directions of an action, it is able to partially retain its temporal structure by applying a windowing scheme. The descriptor, together with a standard classifier, outperforms several state-of-the-art techniques on many well-known datasets.

==> tex/bibliography.tex <==
% !TeX spellcheck = en_US

%\bibitem{KargerD}
%Karger D. Ruhl M. Simple efficient load balancing algorithms for
%peer-to-peer systems. In: Proceedings of Sixteenth Annual ACM
%Symposium on Parallelism in Algorithm and Architectures. 2004,
%36--40

%\bibitem{Yao2011}
%Yao, Angela, Juergen Gall, Gabriele Fanelli, and Luc J. Van Gool. Does Human Action Recognition Benefit from Pose Estimation?. In BMVC, vol. 3, p. 6. 2011.
%  
  
%\bibitem{Mohammad2013}  
%Gowayyed, Mohammad A., Marwan Torki, Mohamed E. Hussein, and Motaz El-Saban. "Histogram of oriented displacements (HOD): describing trajectories of human joints for action recognition." In Proceedings of the Twenty-Third international joint conference on Artificial Intelligence, pp. 1351-1357. AAAI Press, 2013.
